CCMNet: Leveraging Calibrated Color Correction Matrices for Cross-Camera Color Constancy

Computational color constancy, or white balancing, is a key module in a camera's image signal processor (ISP) that corrects color casts from scene lighting. Because this operation occurs in the camera-specific raw color space, white balance algorithms must adapt to different cameras. This paper introduces a learning-based method for cross-camera color constancy that generalizes to new cameras without retraining. Our method leverages pre-calibrated color correction matrices (CCMs) available on ISPs that map the camera's raw color space to a standard space (e.g., CIE XYZ). Our method uses these CCMs to transform predefined illumination colors (i.e., along the Planckian locus) into the test camera's raw space. The mapped illuminants are encoded into a compact camera fingerprint embedding (CFE) that enables the network to adapt to unseen cameras. To prevent overfitting due to limited cameras and CCMs during training, we introduce a data augmentation technique that interpolates between cameras and their CCMs. Experimental results across multiple datasets and backbones show that our method achieves state-of-the-art cross-camera color constancy while remaining lightweight and relying only on data readily available in camera ISPs.

==> tab/model_size.tex <==
\begin{table}[h]
\centering
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
 & C5 ($m = 7$) & C5 ($m = 9$) & CCMNet (w/ CFE) & CCMNet (w/o CFE) \\
\midrule \midrule
Size (MB) & 1.64 & 2.09 & 2.59 & \textbf{1.05} \\
\bottomrule
\end{tabular}}
\caption{Comparison of model sizes.}
\label{tab:model_sizes}
\end{table}
